Dynamic pricing and assortment under a contextual MNL demand

We consider dynamic multi-product pricing and assortment problems under an unknown demand over T periods, where in each period, the seller decides on the price for each product or the assortment of products to offer to a customer who chooses according to an unknown Multinomial Logit Model (MNL). Such problems arise in many applications, including online retail and advertising. We propose a randomized dynamic pricing policy based on a variant of the Online Newton Step algorithm (ONS) that achieves a $O(d\sqrt{T}\log(T))$ regret guarantee under an adversarial arrival model. We also present a new optimistic algorithm for the adversarial MNL contextual bandits problem, which achieves a better dependency than the state-of-the-art algorithms in a problem-dependent constant $\kappa_2$ (potentially exponentially small). Our regret upper bound scales as $\tilde{O}(d\sqrt{\kappa_2 T}+ \log(T)/\kappa_2)$, which gives a stronger bound than the existing $\tilde{O}(d\sqrt{T}/\kappa_2)$ guarantees.

==> abstract.tex <==
\begin{abstract}

We consider dynamic multi-product pricing and assortment problems under an unknown demand over T periods, where in each period, the seller decides on the price for each product or the assortment of products to offer to a customer who chooses according to an unknown Multinomial Logit Model (MNL). Such a problem arises in many applications including online retail and advertising. We propose a randomized dynamic pricing policy based on a variant of the Online Newton Step algorithm (ONS) which achieves a $O(\sqrt{T}\log(T))$ regret guarantee when the feature vectors are adversarially chosen by nature and the price sensitivities are feature-dependent. We also present a new optimistic algorithm for the adversarial MNL contextual bandits problem which achieve a better dependency than the existing algorithms in a problem dependent constant which make take exponential values.


We consider the problem faced by a firm which has to sell a set of highly-differentiated products over a time horizon of T periods. At each period, the firm has to price multiple products to sell them to its customers. Customers make purchases according to the common Multinomial Logit Model (MNL), where the value of each product depends on a vector of features associated with it and the price posted by the seller. The firm receives at each period the features of the products under consideration for sale but does not initially know the values corresponding to these features. However, it can learn it through the outcomes of the previous sales. This model is motivated by applications such as online marketplaces. We propose a randomized dynamic pricing policy based on Online Newton step algorithm (ONS) which achieves a $O(\sqrt{T}\log(T))$ regret guarantee when the feature vectors are adversarially chosen by nature and the price sensitivity are features-dependant. We also show that our pricing policy achieves similar regret performance for more general value models when the firm has to price a single product at each period. 
\end{abstract}
